GraphCare: Enhancing Healthcare Predictions with Personalized Knowledge Graphs

Clinical predictive models often rely on patients' electronic health records (EHR), but integrating medical knowledge to enhance predictions and decision-making is challenging. This is because personalized predictions require personalized knowledge graphs (KGs), which are difficult to generate from patient EHR data. To address this, we propose \textsc{GraphCare}, an open-world framework that uses external KGs to improve EHR-based predictions. Our method extracts knowledge from large language models (LLMs) and external biomedical KGs to build patient-specific KGs, which are then used to train our proposed Bi-attention AugmenTed (BAT) graph neural network (GNN) for healthcare predictions. On two public datasets, MIMIC-III and MIMIC-IV, \textsc{GraphCare} surpasses baselines in four vital healthcare prediction tasks: mortality, readmission, length of stay (LOS), and drug recommendation. On MIMIC-III, it boosts AUROC by 17.6\% and 6.6\% for mortality and readmission, and F1-score by 7.9\% and 10.8\% for LOS and drug recommendation, respectively. Notably, \textsc{GraphCare} demonstrates a substantial edge in scenarios with limited data availability. Our findings highlight the potential of using external KGs in healthcare prediction tasks and demonstrate the promise of \textsc{GraphCare} in generating personalized KGs for promoting personalized medicine.

==> figures/pat_repre_perf.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/patient_repre_perf.pdf}
    
    \caption{\textbf{Performance of healthcare predictions with three types of patient representations}: (1) \textbf{graph} -  patient graph embedding obtained through mean pooling of node embedding; (2) \textbf{node} - patient node embedding connected to the direct EHR node; (3) \textbf{joint} - embedding concatenated by (1) and (2).}
    \label{fig:pat_repre_perf}
\end{figure}

==> figures/perf_AUROC_vis.tex <==
\begin{figure}[!tp]
    \vspace{-2ex}
    \centering
    \includegraphics[width=\linewidth]{figures/perf_vis.pdf}
    \caption{\textbf{Performance of AUROC for all models across all tasks/datasets}. We highlight the performance of our proposed \textsc{GraphCare} w/ \texttt{BAT} with green circles.}
    \label{fig:p Weerf_vis}
    \vspace{-3ex}
\end{figure}

==> tables/bi_att_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[H]
\caption{\textbf{Ablation study}. We measure the AUROC (\%) for each task. $\alpha$, $\beta$ and $W_{\mathcal{R}}$ are node-level, visit-level attention, and edge weight, respectively. We highlight the best results on both \bluebox{\textbf{MIMIC-III}} and \yellowbox{\textbf{MIMIC-IV}}.}
\centering
% \setlength{\tabcolsep}{3.9pt}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{l|ccc|cccc}
\toprule   
\#&$\alpha$    & $\beta$   & $W_{\mathcal{R}}$     & \textbf{Mortality}     & \textbf{Readmission}    & \textbf{LOS}  & \textbf{Drug Rec.} \\
\midrule
1 &\xmark &\xmark&\xmark   & $66.9/70.5$   & $66.7/66.2$   & $79.2/79.0$  & $94.5/94.1$   \\
2 &\cmark &\xmark&\xmark   & $69.1/71.4$   & $68.2/66.9$   & $80.0/79.7$  & $94.9/94.3$    \\
3 &\xmark &\cmark&\xmark   & $67.3/71.0$   & $67.0/66.7$   & $79.4/79.2$  & $94.8/94.2$   \\
4 &\cmark &\xmark&\cmark   & $69.4/71.4$   & $68.3/66.8$   & \bluebox{\textbf{80.3}}$/79.6$  & \bluebox{\textbf{95.1}}$/94.4$   \\
5 &\xmark &\cmark&\cmark   & $68.0/71.3$   & $67.3/66.3$   & $79.5/79.3$  & $94.8/94.2$    \\
6 &\cmark &\cmark&\xmark   & $69.1/71.7$   & $68.4/$\yellowbox{\textbf{67.2}}    & $80.0/$\yellowbox{\textbf{80.4}}  & $95.0/94.5$    \\
7 &\cmark &\cmark&\cmark   & \bluebox{\textbf{69.6}}$/$\yellowbox{\textbf{71.8}}   & \bluebox{\textbf{68.9}}$/67.1$  & $80.2/80.1$  & \bluebox{\textbf{95.1}}$/$\yellowbox{\textbf{94.6}}    \\
\bottomrule
\end{tabular}
}
\label{tb:bi_att_ablation}
\end{table}

                                





==> tables/gnn_compare.tex <==
\begin{table}[!h]
\centering
\caption{\textbf{Performance comparison of GNN models.} In addition to GAT and GIN, we further compare our proposed graph neural network \texttt{BAT} to two powerful graph transformer models: EGT (Hussain, et al. KDD'22), and GraphGPS (Rampášek, Ladislav, et al. NeurIPS'22). We highlight top- \textcolor{red}{\textbf{1}}, \textcolor{teal}{2}, \textcolor{blue}{3} results.}
\label{tb:gnn_compare}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\midrule
& \multicolumn{4}{c}{\textbf{Task 1: Mortality Prediction}}
\\
\multicolumn{1}{c}{Model}
& \multicolumn{2}{c}{\textbf{MIMIC-III}}
& \multicolumn{2}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUPRC} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AUROC} 
\\

\midrule
GAT
& $0.138_{(0.009)}$ 
& $0.666_{(0.011)}$      
& $\textcolor{blue}{0.049_{(0.001)}}$
& $0.705_{(0.010)}$

\\
GIN       
& $0.136_{(0.004)}$
& $0.663_{(0.013)}$   
& $\textcolor{teal}{0.052_{(0.001)}}$
& $0.708_{(0.008)}$

\\
EGT
& $\textcolor{blue}{0.145_{(0.005)}}$
& $\textcolor{blue}{0.682_{(0.010)}}$
& $\textcolor{teal}{0.052_{(0.001)}}$
& $\textcolor{blue}{0.710_{(0.007)}}$
\\
GraphGPS
& $\textcolor{teal}{0.148_{(0.002)}}$
& $\textcolor{teal}{0.683_{(0.009)}}$
& $\textcolor{red}{\mathbf{0.054_{(0.001)}}}$
& $\textcolor{teal}{0.713_{(0.011)}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.157_{(0.004)}} }$      
& $\textcolor{red}{\mathbf{0.696_{(0.007)}} }$  
& $\textcolor{teal}{0.052_{(0.001)} }$
& $\textcolor{red}{\mathbf{0.718_{(0.007)}} }$

\\
\midrule
\midrule
& \multicolumn{4}{c}{\textbf{Task 2: Readmission Prediction}}
\\
\multicolumn{1}{c}{Model}
& \multicolumn{2}{c}{\textbf{MIMIC-III}}
& \multicolumn{2}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUPRC} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AUROC}
\\

\midrule
GAT
& $0.709_{(0.009)}$                     
& $0.673_{(0.008)}$  
& $0.674_{(0.004)}$
& $0.666_{(0.003)}$
\\
GIN       
& $0.708_{(0.008)}$   
& $0.675_{(0.004)}$  
& $\textcolor{red}{\mathbf{0.683_{(0.004)}}}$
& $\textcolor{teal}{0.670_{(0.003)}}$
\\
EGT
& $\textcolor{teal}{0.720_{(0.005)}}$ 
& $\textcolor{teal}{0.681_{(0.001)}}$
& $\textcolor{blue}{0.677_{(0.002)}}$
& $\textcolor{blue}{0.668_{(0.005)}}$
\\
GraphGPS
& $\textcolor{blue}{0.714_{(0.007)}}$ 
& $\textcolor{blue}{0.680_{(0.006)}}$
& $0.675_{(0.005)}$
& $\textcolor{blue}{0.668_{(0.010)}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.726_{(0.005)}}}$
& $\textcolor{red}{\mathbf{0.689_{(0.004)}}}$  
& $\textcolor{teal}{0.680_{(0.002)}}$
& $\textcolor{red}{\mathbf{0.671_{(0.004)}}}$
\\
\midrule
\midrule
& \multicolumn{4}{c}{\textbf{Task 3: Length of Stay Prediction}}
\\
% \cmidrule(lr){2-9}
\multicolumn{1}{c}{Model}
& \multicolumn{4}{c}{\textbf{MIMIC-III}}
\\
\cmidrule(lr){2-5}
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUROC}
& \textbf{Cohen's Kappa}
& \textbf{Accuracy}
& \textbf{F1-score}
\\
\midrule
GAT
& $ 0.789_{(0.003)}$
& $ 0.265_{(0.003)}$
& $ 0.405_{(0.002)}$
& $ 0.351_{(0.003)}$
\\
GIN
& $ 0.790_{(0.002)}$
& $ 0.268_{(0.003)}$
& $ \textcolor{blue}{0.408_{(0.003)}}$
& $ 0.353_{(0.004)}$
\\
EGT
& $\textcolor{teal}{0.797_{(0.001)}}$
& $\textcolor{teal}{0.274_{(0.002)}}$
& $\textcolor{teal}{0.415_{(0.003)}}$
& $\textcolor{teal}{0.363_{(0.003)}}$
\\
GraphGPS
& $\textcolor{blue}{0.794_{(0.002)}}$
& $\textcolor{blue}{0.270_{(0.003)}}$
& $\textcolor{teal}{0.415_{(0.003)}}$
& $\textcolor{blue}{0.362_{(0.005)}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.802_{(0.002)}}}$
& $\textcolor{red}{\mathbf{0.285_{(0.002)}}}$
& $\textcolor{red}{\mathbf{0.418_{(0.002)}}}$
& $\textcolor{red}{\mathbf{0.366_{(0.003)}}}$

\\
\midrule
\multicolumn{1}{c}{Model}
& \multicolumn{4}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-5} 
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUROC}
& \textbf{Cohen's Kappa}
& \textbf{Accuracy}
& \textbf{F1-score}
\\
\midrule
GAT
& $0.792_{(0.002)}$
& $0.261_{(0.003)}$
& $0.355_{(0.001)}$
& $0.321_{(0.003)}$
\\
GIN
& $\textcolor{blue}{0.795_{(0.002)}}$
& $0.261_{(0.002)}$
& $\textcolor{teal}{0.364_{(0.003)}}$
& $0.324_{(0.002)}$
\\
EGT
& $\textcolor{teal}{0.798_{(0.003)}}$
& $\textcolor{blue}{0.266_{(0.001)}}$
& $\textcolor{blue}{0.357_{(0.002)}}$
& $\textcolor{blue}{0.325_{(0.002)}}$
\\
GraphGPS
& $\textcolor{red}{\mathbf{0.801_{(0.003)}}}$
& $\textcolor{red}{\mathbf{0.270_{(0.004)}}}$
& $\textcolor{red}{\mathbf{0.366_{(0.003)}}}$
& $\textcolor{red}{\mathbf{0.331_{(0.004)}}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.801_{(0.003)}}}$
& $\textcolor{teal}{0.268_{(0.003)}}$
& $\textcolor{teal}{0.364_{(0.003)}}$
& $\textcolor{teal}{0.328_{(0.002)}}$

\\
\midrule
\midrule
& \multicolumn{4}{c}{\textbf{Task 4: Drug Recommendation}}
\\
% \cmidrule(lr){2-9}
\multicolumn{1}{c}{Model}
& \multicolumn{4}{c}{\textbf{MIMIC-III}}
\\
\cmidrule(lr){2-5} 
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUPRC}
& \textbf{AUROC}
& \textbf{F1-score}
& \textbf{Jaccard}
\\
\midrule

GAT
& $0.778_{(0.002)}$         
& $\textcolor{blue}{0.948_{(0.001)}}$          
& $0.636_{(0.004)}$                     
& $0.482_{(0.004)}$  
\\
GIN
& $\textcolor{blue}{0.782_{(0.001)}}$
& $0.947_{(0.001)}$ 
& $0.636_{(0.004)}$
& $0.479_{(0.003)}$
\\
EGT
& $0.780_{(0.002)}$
& $0.947_{(0.001)}$ 
& $\textcolor{blue}{0.644_{(0.003)}}$ 
& $\textcolor{teal}{0.488_{(0.004)}}$
\\
GraphGPS
& $\textcolor{teal}{0.784_{(0.001)}}$
& $\textcolor{teal}{0.950_{(0.002)}}$ 
& $\textcolor{teal}{0.647_{(0.002)}}$ 
& $\textcolor{blue}{0.484_{(0.003)}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.792_{(0.002)}}}$
& $\textcolor{red}{\mathbf{0.951_{(0.001)}}}$
& $\textcolor{red}{\mathbf{0.652_{(0.002)}}}$
& $\textcolor{red}{\mathbf{0.491_{(0.003)}}}$
\\
\midrule

\multicolumn{1}{c}{Model}
& \multicolumn{4}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-5}
\multicolumn{1}{c}{(w/ \texttt{GraphCare})}
& \textbf{AUPRC}
& \textbf{AUROC}
& \textbf{F1-score}
& \textbf{Jaccard}
\\
\midrule
GAT
& $\textcolor{blue}{0.747_{(0.005)}}$
& $\textcolor{teal}{0.944_{(0.003)}}$
& $0.604_{(0.003)}$
& $0.457_{(0.004)}$
\\
GIN
& $\textcolor{teal}{0.748_{(0.003)}}$
& $\textcolor{red}{\mathbf{0.946_{(0.001)}}}$
& $0.606_{(0.004)}$
& $\textcolor{teal}{0.461_{(0.004)}}$
\\
EGT
& $0.746_{(0.002)}$
& $\textcolor{teal}{0.944_{(0.001)}}$
& $\textcolor{blue}{0.610_{(0.002)}}$
& $\textcolor{blue}{0.458_{(0.002)}}$
\\
GraphGPS
& $\textcolor{teal}{0.748_{(0.003)}}$
& $\textcolor{teal}{0.944_{(0.002)}}$
& $\textcolor{teal}{0.612_{(0.003)}}$
& $\textcolor{red}{\mathbf{0.463_{(0.004)}}}$
\\
\texttt{BAT}
& $\textcolor{red}{\mathbf{0.752_{(0.001)}}}$
& $\textcolor{red}{\mathbf{0.946_{(0.001)}}}$
& $\textcolor{red}{\mathbf{0.615_{(0.003)}}}$
& $\textcolor{red}{\mathbf{0.463_{(0.002)}}}$
\\
\bottomrule
\end{tabular}
}
\vskip -3ex
\end{table}

==> tables/kg_compare.tex <==
\begin{table}[ht]
\caption{\textsc{GraphCare}'s performance by different KGs on MIMIC-III.}
\centering
\resizebox{0.9\textwidth}{!}{\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{KG} & \multicolumn{2}{c}{\textbf{Mortality}} & \multicolumn{2}{c}{\textbf{Readmission}} & \multicolumn{2}{c}{\textbf{LOS}} & \multicolumn{2}{c}{\textbf{Drug Rec.}} \\ 
  & AUPRC & AUROC & AUPRC & AUROC & F1-score & AUROC & F1-score & AUROC \\
  \midrule
GPT-KG              & \textbf{15.7} & \textbf{69.6} & 72.6          & \textbf{68.9} & \textbf{36.6} & \textbf{80.2} & \textbf{65.2} & \textbf{95.1} \\ 
UMLS-KG             & 14.1          & 66.6          & 70.1          & 66.3 & 35.3          & 78.8          & 63.5          & 94.3 \\ 
GPT-UMLS-KG         & 15.4          & 69.3          & \textbf{72.7} & 68.8 & \textbf{36.6} & 79.9          & 64.9          & 95.0 \\ 
\bottomrule
\end{tabular}
}

% \vspace{1em}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{KG} & \multicolumn{2}{c}{\textbf{LOS}} & \multicolumn{2}{c}{\textbf{Drug Rec.}} \\
%   & F1-score & AUROC & F1-score & AUROC \\ 
%  \midrule
% GPT-KG              & \textbf{36.6} & \textbf{80.2} & \textbf{65.2} & \textbf{95.3} \\ 
% UMLS-KG             & 35.3          & 78.8          & 63.5          & 94.3 \\ 
% GPT-UMLS-KG         & \textbf{36.6} & 79.9          & 64.9          & 95.0 \\ 
% \bottomrule
% \end{tabular}}

\label{tb:kg_compare}
\end{table}

==> tables/kg_ratio.tex <==
\begin{table}[H]
\centering
\caption{[Running experiment on different KGs, will use barchart for visualization] \textbf{The performance of \textsc{GraphCare} with different KG sizes.} All KGs are randomly sampled from the global KG while keeping the nodes of EHR medical concepts fixed. For each ratio, we report the average nodes/edges of the patient's personalized KG as well as the performance across four tasks on MIMIC-III.}
\begin{minipage}{.5\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multicolumn{9}{c}{\textbf{Feature: Condition + Procedure + Drug}} \\
\midrule
\textbf{KG Ratio} & & \textbf{0} & \textbf{0.1} & \textbf{0.3} & \textbf{0.5} & \textbf{0.7} & \textbf{0.9} & \textbf{1.0} \\
\midrule
\multicolumn{2}{l}{Nodes/pat.} & 242 & 362 & 618 & 883 & 1113 & 1359 & 1479 \\
\multicolumn{2}{l}{Edges/pat.} & 288 & 485 & 886 & 1296 & 1690 & 2170 & 2374 \\
\midrule
\multirow{2}{*}{\textbf{MT.}} & AUPRC & 0.13 & 0.13 & 0.14 & 0.15 & 0.15 & 0.15 & \textbf{0.16} \\
 & AUROC & 0.64 & 0.65 & 0.67 & 0.68 & 0.68 & 0.69 & \textbf{0.70} \\
\multirow{2}{*}{\textbf{RA.}} & AUPRC & 0.70 & 0.71 & 0.71 & 0.71 & 0.72 & 0.72 & \textbf{0.73} \\
 & AUROC & 0.67 & 0.68 & 0.68 & 0.68 & \textbf{0.69} & \textbf{0.69} & \textbf{0.69} \\
\bottomrule
\end{tabular}
}
\label{tb:kg_ratio1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multicolumn{9}{c}{\textbf{Feature: Condition + Procedure}} \\
\midrule
\textbf{KG Ratio} & & \textbf{0} & \textbf{0.1} & \textbf{0.3} & \textbf{0.5} & \textbf{0.7} & \textbf{0.9} & \textbf{1.0} \\
\midrule
\multicolumn{2}{l}{Nodes/pat.} & 15 & 47 & 139 & 221 & 317 & 401 & 447 \\
\multicolumn{2}{l}{Edges/pat.} & 6 & 25 & 140 & 261 & 398 & 599 & 666 \\
\midrule
\multirow{2}{*}{\textbf{LOS}} & AUROC & 0.77 & 0.78 & 0.78 & 0.79 & 0.79 & \textbf{0.80} & \textbf{0.80} \\
 & F1 & 0.34 & 0.35 & 0.35 & 0.35 & 0.36 & 0.36 & \textbf{0.37} \\
\multirow{2}{*}{\textbf{Drug.}} & AUROC & 0.94 & 0.94 & 0.94 & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} & \textbf{0.95} \\
 & F1 & 0.61 & 0.62 & 0.63 & 0.64 & 0.64 & \textbf{0.65} & \textbf{0.65} \\
\bottomrule
\end{tabular}
}
\label{tb:kg_ratio}
\end{minipage}
\end{table}



==> tables/kg_rocauc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{wraptable}{l}{0pt}
\resizebox{0.6\textwidth}{!}{
% \setlength{\tabcolsep}{3.9pt}
\begin{tabular}{lcccc}
\toprule   
       & \textbf{Mortality}     & \textbf{Readmission}    & \textbf{Len. of Stay}  & \textbf{Drug Rec.} \\
KG & (PR, ROC)-AUC      & (PR, ROC)-AUC  & (C.K., AUROC)   &(PR, ROC)-AUC
\\
\midrule
\textbf{UMLS-KG}     & $(0.123, 0.639)$       & $(0.678, 0.633)$      & $(0.255, 0.778)$  & $(0.764, 0.943)$ \\
\textbf{GPT-KG}      & $(\liyellowtbox{\textbf{0.152}} , \liyellowtbox{\textbf{0.692}})$     & $(\liyellowtbox{\textbf{0.714}}, \liyellowtbox{\textbf{0.686}})$      & $(0.273, \liyellowtbox{\textbf{0.794}})$   & $(\liyellowtbox{\textbf{0.788}}, 0.951)$   \\
\textbf{Combined-KG}    & $(0.142, 0.669)$   & $(0.707, 0.679)$   & $(\liyellowtbox{\textbf{0.276}}, 0.786)$   & $(0.787, \liyellowtbox{\textbf{0.953}})$   \\
\bottomrule
\end{tabular}
}
\caption{Performanace on MIMIC-III with different KGs. C.K. denotes Conhen's Kappa. UMLS-KG and GPT-KG are the KGs composed by $G^{e}_{\mathrm{sub}}$ and $G^{e}_{\mathrm{LLM}}$ (\S\ref{subsec:ehr_graph}) correspondingly. "Combined-KG" is the KG combined by both KGs. The best results are \liyellowtbox{\textbf{highlighted}}.}

\label{tb:kg_AUROC}
\end{wraptable}
                                





==> tables/performance_comparison.tex <==
\begin{table*}[!tp]
\centering
\caption{\textbf{Performance comparison of four prediction tasks on MIMIC-III/MIMIC-IV.} We report the average performance and the standard deviation (in bracket) of each model over 100 runs for MIMIC-III and 50 runs for MIMIC-IV. The best results are \textbf{highlighted} for both datasets.}
\label{tb:perf_compare}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{4}{c}{\textbf{Task 1: Mortality Prediction}}
& \multicolumn{4}{c}{\textbf{Task 2: Readmission Prediction}}
\\
Model
& \multicolumn{2}{c}{\textbf{MIMIC-III}}
& \multicolumn{2}{c}{\textbf{MIMIC-IV}}
& \multicolumn{2}{c}{\textbf{MIMIC-III}}
& \multicolumn{2}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \textbf{AUPRC} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AUROC}
\\
\midrule
GRU           
& $0.12_{(0.01)}$ 
& $0.61_{(0.01)}$ 
& $0.04_{(0.00)}$ 
& $0.69_{(0.01)}$    

& $0.68_{(0.00)}$ 
&$0.65_{(0.01)}$ 
&$0.66_{(0.00)}$ 
&$0.66_{(0.00)}$
\\

Transformer   
& $0.10_{(0.01)}$    
& $0.57_{(0.01)}$
& $0.03_{(0.00)}$
& $0.65_{(0.01)}$

& $0.67_{(0.01)}$
& $0.64_{(0.01)}$
& $0.66_{(0.00)}$
& $0.65_{(0.00)}$
\\
                                                
RETAIN        
& $0.10_{(0.01)}$     
& $0.59_{(0.01)}$  
& $0.04_{(0.00)}$
& $0.65_{(0.02)}$

& $0.65_{(0.01)}$
& $0.64_{(0.01)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$

\\

GRAM
& $0.11_{(0.01)}$
& $0.60_{(0.01)}$
& $0.04_{(0.00)}$
& $0.67_{(0.01)}$

& $0.67_{(0.01)}$
& $0.64_{(0.00)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
\\

Deepr
& $0.13_{(0.01)}$
& $0.61_{(0.00)}$
& $0.04_{(0.00)}$
& $0.69_{(0.01)}$

& $0.69_{(0.01)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
& $0.65_{(0.00)}$
\\

AdaCare
& $0.11_{(0.00)}$
& $0.58_{(0.01)}$
& $\mathbf{0.05_{(0.00)}}$
& $0.69_{(0.01)}$

& $0.68_{(0.01)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
\\

GRASP
& $0.10_{(0.01)}$
& $0.59_{(0.01)}$
& $\mathbf{0.05_{(0.00)}}$
& $0.68_{(0.01)}$

& $0.69_{(0.00)}$
& $0.66_{(0.01)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
\\

StageNet
& $0.12_{(0.00)}$
& $0.62_{(0.01)}$
& $0.04_{(0.00)}$
& $0.70_{(0.01)}$

& $0.69_{(0.01)}$
& $0.67_{(0.00)}$
& $0.66_{(0.00)}$
& $0.66_{(0.00)}$
\\
\midrule

\texttt{GraphCare} w/ GAT
& $0.14_{(0.01)}$ 
& $0.67_{(0.01)}$      
& $0.05_{(0.00)}$
& $0.71_{(0.01)}$

& $0.71_{(0.01)}$                     
& $0.67_{(0.01)}$  
& $0.67_{(0.00)}$
& $\mathbf{0.67_{(0.00)}}$
\\
\texttt{GraphCare} w/ GIN       
& $0.14_{(0.00)}$
& $0.66_{(0.01)}$   
& $\mathbf{0.05_{(0.00)}}$
& $0.71_{(0.01)}$

& $0.71_{(0.01)}$   
& $0.68_{(0.00)}$  
& $\mathbf{0.68_{(0.00)}}$
& $\mathbf{0.67_{(0.00)}}$

\\
\texttt{GraphCare} w/ \texttt{BAT}
& $\mathbf{0.16_{(0.00)}} $      
& $\mathbf{0.70_{(0.01)}} $  
&$\mathbf{0.05_{(0.00)}} $
&$\mathbf{0.72_{(0.01)}} $

& $\mathbf{0.73_{(0.01)}} $
& $\mathbf{0.69_{(0.00)}} $  
& $\mathbf{0.68_{(0.00)}}$
& $\mathbf{0.67_{(0.00)}} $
\\
\midrule
& \multicolumn{8}{c}{\textbf{Task 3: Length of Stay Prediction}}
\\
% \cmidrule(lr){2-9}
Model
& \multicolumn{4}{c}{\textbf{MIMIC-III}}
& \multicolumn{4}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \textbf{AUROC}
& \textbf{Kappa}
& \textbf{Accuracy}
& \textbf{F1}
& \textbf{AUROC}
& \textbf{Kappa}
& \textbf{Accuracy}
& \textbf{F1}
\\
\midrule
GRU
& $ 0.78_{(0.00)} $
& $ 0.26_{(0.00)} $
& $ 0.40_{(0.00)} $
& $ 0.35_{(0.01)} $

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $0.35_{(0.00)}$
& $0.32_{(0.00)}$
\\
Transformer
& $ 0.78_{(0.00)}$
& $ 0.25_{(0.00)}$
& $ 0.40_{(0.00)}$
& $ 0.35_{(0.00)}$

& $0.78_{(0.00)}$
& $0.25_{(0.00)}$
& $0.34_{(0.00)}$
& $0.31_{(0.00)}$
\\
RETAIN
& $ 0.78_{(0.00)}$
& $ 0.26_{(0.00)}$
& $ 0.41_{(0.00)}$
& $ 0.35_{(0.00)}$

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $\mathbf{0.36_{(0.00)}}$
& $0.32_{(0.00)}$
\\

GRAM
& $0.78_{(0.00)}$
& $0.26_{(0.00)}$
& $0.40_{(0.00)}$
& $0.34_{(0.00)}$

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $0.35_{(0.00)}$
& $0.32_{(0.00)}$
\\

Deepr
& $0.78_{(0.00)}$
& $0.25_{(0.00)}$
& $0.40_{(0.01)}$
& $0.35_{(0.00)}$

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $\mathbf{0.36_{(0.00)}}$
& $0.32_{(0.00)}$
\\

StageNet
& $0.78_{(0.00)}$
& $0.25_{(0.00)}$
& $0.40_{(0.00)}$
& $0.34_{(0.00)}$

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $0.35_{(0.00)}$
& $0.31_{(0.00)}$
\\

\midrule
\texttt{GraphCare} w/ GAT
& $ 0.79_{(0.00)}$
& $ 0.27_{(0.00)}$
& $ 0.41_{(0.00)}$
& $ 0.35_{(0.00)}$

& $0.79_{(0.00)}$
& $0.26_{(0.00)}$
& $\mathbf{0.36_{(0.00)}}$
& $0.32_{(0.00)}$
\\
\texttt{GraphCare} w/ GIN
& $ 0.79_{(0.00)}$
& $ 0.27_{(0.00)}$
& $ 0.41_{(0.00)}$
& $ 0.35_{(0.00)}$

& $\mathbf{0.80_{(0.00)}}$
& $0.26_{(0.00)}$
& $\mathbf{0.36_{(0.00)}}$
& $0.32_{(0.00)}$
\\
\texttt{GraphCare} w/ \texttt{BAT}
& $\mathbf{0.80_{(0.00)}}$
& $\mathbf{0.29_{(0.00)}}$
& $\mathbf{0.42_{(0.00)}}$
& $\mathbf{0.37_{(0.00)}}$

& $\mathbf{0.80_{(0.00)}}$
& $\mathbf{0.27_{(0.00)}}$
& $\mathbf{0.36_{(0.00)}}$
& $\mathbf{0.33_{(0.00)}}$

\\
\midrule
& \multicolumn{8}{c}{\textbf{Task 4: Drug Recommendation}}
\\
% \cmidrule(lr){2-9}
Model
& \multicolumn{4}{c}{\textbf{MIMIC-III}}
& \multicolumn{4}{c}{\textbf{MIMIC-IV}}
\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \textbf{AUPRC}
& \textbf{AUROC}
& \textbf{F1}
& \textbf{Jaccard}
& \textbf{AUPRC}
& \textbf{AUROC}
& \textbf{F1}
& \textbf{Jaccard}
\\
\midrule
GRU
& $0.77_{(0.00)}$
& $0.94_{(0.00)}$
& $0.62_{(0.00)}$
& $0.48_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.44_{(0.00)}$
\\

Transformer
& $0.76_{(0.00)}$
& $0.94_{(0.00)}$
& $0.62_{(0.00)}$
& $0.47_{(0.00)}$

& $0.71_{(0.00)}$
& $0.93_{(0.00)}$
& $0.56_{(0.00)}$
& $0.40_{(0.00)}$
\\

RETAIN
& $0.77_{(0.00)}$
& $0.94_{(0.00)}$
& $0.64_{(0.00)}$
& $\mathbf{0.49_{(0.00)}}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.45_{(0.00)}$
\\

GRAM
& $0.77_{(0.00)}$
& $0.94_{(0.00)}$
& $0.63_{(0.00)}$
& $0.48_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.45_{(0.00)}$
\\

Deepr
& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.45_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.59_{(0.00)}$
& $0.44_{(0.00)}$
\\

StageNet
& $0.74_{(0.00)}$
& $0.93_{(0.00)}$
& $0.61_{(0.00)}$
& $0.46_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.45_{(0.00)}$
\\

SafeDrug
& $0.68_{(0.00)}$
& $0.91_{(0.00)}$
& $0.47_{(0.00)}$
& $0.32_{(0.00)}$

& $0.66_{(0.01)}$
& $0.92_{(0.00)}$
& $0.56_{(0.00)}$
& $0.44_{(0.00)}$
\\

MICRON
& $0.77_{(0.00)}$
& $\mathbf{0.95_{(0.00)}}$
& $0.63_{(0.00)}$
& $0.48_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.59_{(0.00)}$
& $0.44_{(0.00)}$
\\

GAMENet
& $0.76_{(0.00)}$
& $0.94_{(0.00)}$
& $0.62_{(0.00)}$
& $0.47_{(0.00)}$

& $0.74_{(0.00)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $0.45_{(0.00)}$
\\

MoleRec
& $0.70_{(0.00)}$
& $0.92_{(0.00)}$
& $0.58_{(0.00)}$
& $0.43_{(0.00)}$

& $0.69_{(0.00)}$
& $0.92_{(0.00)}$
& $0.56_{(0.00)}$
& $0.41_{(0.00)}$

\\
\midrule

\texttt{GraphCare} w/ GAT
& $0.78_{(0.00)}$         
& $\mathbf{0.95_{(0.00)}}$          
& $0.64_{(0.00)}$                     
& $0.48_{(0.00)}$  

& $0.75_{(0.01)}$
& $0.94_{(0.00)}$
& $0.60_{(0.00)}$
& $\mathbf{0.46_{(0.00)}}$
\\
\texttt{GraphCare} w/ GIN
& $0.78_{(0.00)}$
& $\mathbf{0.95_{(0.00)}}$ 
& $0.64_{(0.00)}$
& $0.48_{(0.00)}$

& $\mathbf{0.75_{(0.00)}}$
& $\mathbf{0.95_{(0.00)}}$
& $0.61_{(0.00)}$
& $\mathbf{0.46_{(0.00)}}$
\\
\texttt{GraphCare} w/ \texttt{BAT}
& $\mathbf{0.79_{(0.00)}}$
& $\mathbf{0.95_{(0.00)}}$
& $\mathbf{0.65_{(0.00)}}$
& $\mathbf{0.49_{(0.00)}}$

& $\mathbf{0.75_{(0.00)}}$
& $\mathbf{0.95_{(0.00)}}$
& $\mathbf{0.62_{(0.00)}}$
& $\mathbf{0.46_{(0.00)}}$
\\
\bottomrule
\end{tabular}
}
\vskip -3ex
\end{table*}
                                




